Symmetry-based quantum algorithms for open-shop scheduling with hard constraints

Encoding hard-constrained optimization problems into a variational quantum algorithm often turns out to be a challenging task. In this work, we provide a solution for the class of open-shop scheduling problems (OSSPs), which we achieve by rigorously employing the symmetries of the classical problem. An established approach for encoding the hard constraints of the closely related traveling salesperson problem (TSP) into mixer Hamiltonians was recently given by Hadfield et al.'s Quantum Alternating Operator Ansatz (QAOA). For the OSSP, which contains TSP as a special case, we show that desired properties of similarly constructed mixers can be directly linked to a purely classical object: the group of feasibility-preserving bit value permutations. We also outline a generic way to construct QAOA-like mixers for these problems. We further propose a new variational quantum algorithm that incorporates the underlying group structure more naturally and, as a proof of principle, implement our new algorithm for a small OSSP instance on an IBM Q System One. Unlike the generic QAOA, our algorithm allows for bounding the amount and the domain of parameters necessary to reach every feasible solution from above: Optimizing at most quadratically many parameters should suffice to reach the optimum with certainty.

==> journalnames.tex <==
% Updated 14 November 2024
%\DeclareOption{}{\gdef\@journalweb{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}}
%% Website Name	%%	% Website Name	%% Full Name	%% Short Name	%% DOI abbr	%% ISSN

%1
\DeclareOption{Acad.Biol.}{\gdef\@journal{acadbiol}\gdef\@journalweb{academia-biology}\gdef\@journalfull{ACADEMIA BIOLOGY}\gdef\@journalfullname{Academia Biology}\gdef\@journalshort{Acad. Biol.}\gdef\@doiabbr{AcadBiol}\gdef\@ISSN{2837-4010}}
%2
\DeclareOption{Acad.Energy.}{\gdef\@journal{acadenergy}\gdef\@journalweb{academia-green-energy}\gdef\@journalfull{ACADEMIA GREEN ENERGY}\gdef\@journalfullname{Academia Green Energy}\gdef\@journalshort{Acad. Energy.}\gdef\@doiabbr{AcadEnergy}\gdef\@ISSN{2998-3665}}
%3
\DeclareOption{Acad.Eng.}{\gdef\@journal{acadeng}\gdef\@journalweb{academia-engineering}\gdef\@journalfull{ACADEMIA ENGINEERING}\gdef\@journalfullname{Academia Engineering}\gdef\@journalshort{Acad. Eng.}\gdef\@doiabbr{AcadEng}\gdef\@ISSN{2994-7065}}
%4
\DeclareOption{Acad.Env.Sci.Sust.}{\gdef\@journal{acadenvscisust}\gdef\@journalweb{academia-environmental-sciences-and-sustainability}\gdef\@journalfull{ACADEMIA ENVIRONMENTAL SCIENCES AND SUSTAINABILITY}\gdef\@journalfullname{Academia Environmental Sciences and Sustainability}\gdef\@journalshort{Acad. Env. Sci. Sust.}\gdef\@doiabbr{AcadEnvSciSust}\gdef\@ISSN{2997-6006}}
%5
\DeclareOption{Acad.Mat.Sci.}{\gdef\@journal{acadmatsci}\gdef\@journalweb{academia-materials-science}\gdef\@journalfull{ACADEMIA MATERIALS SCIENCE}\gdef\@journalfullname{Academia Materials Science}\gdef\@journalshort{Acad. Mat. Sci.}\gdef\@doiabbr{AcadMatSci}\gdef\@ISSN{2997-2027}}
%6
\DeclareOption{Acad.Med.}{\gdef\@journal{acadmed}\gdef\@journalweb{academia-medicine}\gdef\@journalfull{ACADEMIA MEDICINE}\gdef\@journalfullname{Academia Medicine}\gdef\@journalshort{Acad. Med.}\gdef\@doiabbr{AcadMed}\gdef\@ISSN{2994-435X}}
%7
\DeclareOption{Acad.Ment.Health.WellB.}{\gdef\@journal{acadmenthealthwellb}\gdef\@journalweb{academia-mental-health-and-well-being}\gdef\@journalfull{ACADEMIA MENTAL HEALTH AND WELL-BEING}\gdef\@journalfullname{Academia Mental Health and Well-Being}\gdef\@journalshort{Acad. Ment. Health WellB.}\gdef\@doiabbr{AcadMentHealthWellB}\gdef\@ISSN{2997-9196}}
%8
\DeclareOption{Acad.Mol.Biol.Genom.}{\gdef\@journal{acadmolbiolgenom}\gdef\@journalweb{academia-molecular-biology-and-genomics}\gdef\@journalfull{ACADEMIA MOLECULAR BIOLOGY AND GENOMICS}\gdef\@journalfullname{Academia Molecular Biology and Genomics}\gdef\@journalshort{Acad. Mol. Biol. Genom.}\gdef\@doiabbr{AcadMolBiolGenom}\gdef\@ISSN{3064-9765}}
%9
\DeclareOption{Acad.NanoSci.Mat.Tech.}{\gdef\@journal{acadnanoscimattech}\gdef\@journalweb{academia-nano-science-materials-technology}\gdef\@journalfull{ACADEMIA NANO: SCIENCE, MATERIALS, TECHNOLOGY}\gdef\@journalfullname{Academia Nano: Science, Materials, Technology}\gdef\@journalshort{Acad. Nano: Sci. Mat. Tech.}\gdef\@doiabbr{AcadNanoSciMatTech}\gdef\@ISSN{3065-9736}}
%10
\DeclareOption{Acad.Nutri.}{\gdef\@journal{acadnutri}\gdef\@journalweb{academia-nutrition-and-dietetics}\gdef\@journalfull{ACADEMIA NUTRITION AND DIETETICS}\gdef\@journalfullname{Academia Nutrition and Dietetics}\gdef\@journalshort{Acad. Nutri.}\gdef\@doiabbr{AcadNutri}\gdef\@ISSN{3067-1345}}
%11
\DeclareOption{Acad.Oncol.}{\gdef\@journal{acadoncol}\gdef\@journalweb{academia-oncology}\gdef\@journalfull{ACADEMIA ONCOLOGY}\gdef\@journalfullname{Academia Oncology}\gdef\@journalshort{Acad. Oncol.}\gdef\@doiabbr{AcadOncol}\gdef\@ISSN{2998-7741}}
%12
\DeclareOption{Acad.Quant.}{\gdef\@journal{acadquant}\gdef\@journalweb{academia-quantum}\gdef\@journalfull{ACADEMIA QUANTUM}\gdef\@journalfullname{Academia Quantum}\gdef\@journalshort{Acad. Quant.}\gdef\@doiabbr{AcadQuant}\gdef\@ISSN{3064-979X}}

\DeclareOption{Acad.Dis.}{\gdef\@journal{acaddis}\gdef\@journalweb{academia-immunity-and- disease}\gdef\@journalfull{ACADEMIA IMMUNITY AND DISEASE}\gdef\@journalfullname{Academia Immunity and Disease}\gdef\@journalshort{Acad. Dis.}\gdef\@doiabbr{AcadDis}\gdef\@ISSN{}}

\DeclareOption{Acad.Drug.}{\gdef\@journal{acaddrug}\gdef\@journalweb{academia-drug-development-and-pharmacotherapy}\gdef\@journalfull{ACADEMIA DRUG DEVELOPMENT AND PHARMACOTHERAPY}\gdef\@journalfullname{Academia Drug Development and Pharmacotherapy}\gdef\@journalshort{Acad. Drug.}\gdef\@doiabbr{AcadDrug}\gdef\@ISSN{}}


\DeclareOption{Acad.AI.}{\gdef\@journal{acadai}\gdef\@journalweb{academia-ai-and-applications}\gdef\@journalfull{ACADEMIA AI AND APPLICATIONS}\gdef\@journalfullname{Academia AI and Applications}\gdef\@journalshort{Acad. AI.}\gdef\@doiabbr{AcadAI}\gdef\@ISSN{}}

\DeclareOption{Acad.Neurosci.BrainRes.}{\gdef\@journal{acadneuroscibrainres}\gdef\@journalweb{academia-neuroscience-and-brain-research}\gdef\@journalfull{ACADEMIA NEUROSCIENCE AND BRAIN RESEARCH}\gdef\@journalfullname{Academia Neuroscience and Brain Research}\gdef\@journalshort{Acad. Neurosci. Brain Res.}\gdef\@doiabbr{AcadNeurosciBrainRes}\gdef\@ISSN{}}





\DeclareOption{nojournal}{\gdef\@journal{acadquant}\gdef\@journalweb{academia-journal}\gdef\@journalfull{Academia Journal}\gdef\@journalfullname{}\gdef\@journalshort{Acad. J.}\gdef\@doiabbr{AcadJ}\gdef\@ISSN{}}

